Direct detection and characterization of exoplanets using imaging Fourier transform spectroscopy

Space-based direct imaging provides prospects for detection and spectral characterization of exoplanets at optical and near-infrared wavelengths. Integral field spectrographs (IFS) have been historically baselined for these mission concepts. However, multiple studies have revealed that detector noise is a serious obstacle for such instruments when observing extremely faint targets such as Earth-like planets. Imaging Fourier transform spectrographs (iFTS) are generally less sensitive to detector noise, and have several other compelling features such as simultaneous imaging and spectroscopy, smaller-format detector requirements, and variable spectral resolution. To date, they have not been studied as options for such missions. In this work, we compare the capabilities of integral field spectrographs and imaging Fourier transform spectrographs to directly obtain spectra from an Earth-like planet using analytic and numerical models. Specifically, we compare the required exposure time to achieve the same signal-to-noise ratio of the two architectures over a range of detector and optical system parameters. We find that for a 6-meter telescope, an IFS outperforms an iFTS at optical wavelengths. In the near-IR, the relative efficiency of an IFS and iFTS depends on the instrument design and detector noise. An iFTS will be more efficient than an IFS if the readout noise of near-IR detector is above 2-3 e-/pix/frame (t_frame=1000s), which correspond to half to one-third of detector noise of the state-of-art. However, if the readout noise is further reduced to below this threshold, the performance of an IFS will experience a substantial improvement and become more efficient. These results motivate consideration of an iFTS as an alternative option for future direct imaging space missions in the near-IR.

==> FTSsimu.tex <==
\begin{figure*}
    \centering  
    \includegraphics[width=0.95\linewidth]{figFTSsinmu.png}
    \caption{Numerical simulations of an iFTS. (a) The input spectra. (b) Exposure time at every optical path difference. We adopt a boxcar apodization function that assigns a constant time at every step. (c) Instrument line spread line function. (d)-(f): The signal, noise and SNR of simulated interferogram. The signal is defined as the mean value obtained from 1000 simulation runs, while the noise is calculated as the standard deviation. The blue curves present the difference between intensity at two outputs, and the orange curves are the sum of intensity at two outputs. The red lines depict analytical models. (g)-(o)  The signal, noise and SNR of output spectra in three different wavenumber ranges.  The signal is also defined as the mean value obtained from 1000 simulation runs, while noise is the standard deviation. Blue lines denote simulated intensity and red lines show the analytical models. }
    \label{fig:FTSsimu}
\end{figure*}

==> IFSsimu.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/figIFSsimu.png}
    \caption{Numerical simulations of an IFS. (a) The input spectra; (b)-(d) the signal, noise and SNR of output spectra. Blue lines are our simulated intensity and spectra. Red lines show the analytical models. 
  }
    \label{fig:IFSsimu}
\end{figure*}

==> appdex_anasnr.tex <==
\section{iFTS SNR derivation}\label{sec:dde}

 In the section, we present analytical derivations of the SNR expressions. We assume the case of a pure planet spectrum $S_{in}(\nu)$ as the input spectrum with detector noise $I_{FTS}$. As described in section 3, the interferogram is the difference between the intensity at two outputs:
\begin{equation}
     I_{\Delta}(\delta) = T(\delta)\sum{S_{in}(\nu)\cos{2\pi \nu \delta}}\Delta \nu 
\end{equation}
The output spectra is 
\begin{equation} \label{eq1}
\begin{split}
S_{o,\rm{FTS}} & = \operatorname{Re}[\sum I_{\Delta}(\delta) e^{-2j\pi \nu \delta}\Delta \delta] \\
               & = \sum I_{\Delta}(\delta) \cos(-2\pi \nu \delta)\Delta \delta  \\
               & =  \frac{S_{in}(\nu) \Delta \nu_{\rm{ILS}} T_{\rm{tot}}}{2}
\end{split}
\end{equation}

The variance  of the output spectra is 
\begin{equation}
    \sigma^{2}[S_{o,\rm{FTS}}] = \sum (I_{\Delta}(\delta)\Delta \delta)^{2} \cos(-2\pi \nu \delta)^{2}
\end{equation}
The $\cos^{2}$ term in above expression can be approximated as 1/2 because it oscillates as $\delta$ much rapidly than $T_{\Delta}(\delta)$ \citep{bennett1999critical}. With this approximation, the spectral noise is independent of wavenumber, i.e. it is white noise.  Another term in above expression $\sum (I_{\Delta}(\delta)\Delta \delta)^{2}$ is the total variance of the interferogram, which is sum of  variance of the interferogram over optical path difference $x$. Thus, we can have the variance of the output spectrum as 
\begin{equation}
\begin{split}
\sigma^{2}[S_{o,\rm{FTS}}] &=\sum \frac{T(\delta)\sum{S_{in}(\nu)\Delta \nu +2 I_{\rm{FTS}}}T(\delta)}{2} \\
                           &= \frac{T_{\rm{tot}}\sum{S_{in}(\nu)\Delta \nu + 2 I_{\rm{FTS}}}T_{\rm{tot}}}{2} 
\end{split}
\end{equation}

Thus the SNR of the output spectrum would be
\begin{equation}
    \rm{SNR_{FTS}}=\frac{S_{in}(\nu) \Delta \nu_{\rm{ILS}} T_{\rm{tot}}}{\sqrt{2[T_{\rm{tot}}\sum{S_{in}(\nu)\Delta \nu + 2 I_{\rm{FTS}}}T_{\rm{tot}}]}}
\end{equation}
 The iFTS SNR is proportional to square root of $\frac{T_{tot}}{2}$: $\rm{SNR_{FTS}}\propto \sqrt{\frac{T_{tot}}{2}}$. In this way, we derive the analytical expressions consistent with the numerical simulations. Our SNR expression is smaller than that from \cite{bennett1999critical} by a a factor of $\sqrt{2}$.

 


==> fig10.tex <==
\begin{figure*}
    \centering
     \includegraphics[width=0.75\linewidth]{figures/lubex_vis.png}
    \caption{Required exposure time ratio between an IFS and an iFTS $\rm{T_{IFS}/{T_{iFTS}}}$ to achieve the same $\rm{S/N}$ with the same resolution for a visible bandpass ($675 - 785 nm$, $R=140$) using HabEx. Top panels: simulation results using Roman CBE level dark current. Bottom panels: simulation results using future dark current rate required by HabEx. The required exposure time ratio changes as functions of target distance, star-planet separation, host star temperature and the number of exozodis.}
    \label{fig:figure10}
\end{figure*}

==> fig11.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/lubex_nir.png}
    \caption{Required exposure time ratio between an IFS and an iFTS $\rm{T_{IFS}/{T_{iFTS}}}$ to achieve the same $\rm{S/N}$s with the same resolution for a NIR bandpass ($1200-1450 - 785 nm$, $R=70$) using HabEx+Sharshade. Top panels: simulation results using JWST level readout noise. Bottom panels: simulation results using future readout noise rate. The required exposure time ratio changes as functions of target distance, star-planet separation, host star temperature and the number of exozodis.}
    \label{fig:figure11}
\end{figure*}

==> fig12.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/LUVOIRB_1.png}
    \caption{Same with Figure~\ref{fig:figure9} but for LUVOIR B.}
    \label{fig:figure12}
\end{figure*}

==> fig13.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/LUVOIRB_2.png}
    \caption{Same with Figure~\ref{fig:figure10} but for LUVOIR B  }
    \label{fig:figure13}
\end{figure*}

==> fig14.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/LUVOIRB_3.png}
    \caption{Same with Figure~\ref{fig:figure11} but for LUVOIR B}
    \label{fig:figure14}
\end{figure*}

==> fig16.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/IFStimevis.png}
    \caption{The exposure time required by an IFS to achieve an SNR of 5 in a visible channel (640 nm-860 nm) as functions of astrophysical parameters including target distance, stellar temperature, star-planet separation, phase angle and phase angle, exozodi level. Top panels: the exposure time were computed with instrument parameters defined in 2a in Table~\ref{tab:so} current detector noise.  Bottom panels: the exposure time were computed with instrument parameters defined in 2b in Table~\ref{tab:so} using future detector noise.}
    \label{fig:figure16}
\end{figure*}

==> fig17.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/IFStimenir.png}
    \caption{The same as figure~\ref{fig:figure16}, but for an NIR channel (1050nm-1250nm) with varied astrophysical parameters.}
    \label{fig:figure17}
\end{figure*}

==> fig7.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.75\linewidth]{Roman_1.png}
    \caption{The required integration time to achieve $\rm{S/N=5}$ for Roman space telescope equipped with an iFTS (red) and an IFS (dark blue) at three spectroscopy bands of Roman. The filter bands are shown as colorful shaded area and every point corresponds to the central wavelength of every band. The target is a 1 $R_{J}$ planet orbiting a Sun-like star at 5.2 AU from 10 pc away. We use 
   two sets of dark current: Roman current best estimate (CBE, solid lines), Roman requirement in the end of life (EOL REQ, dashed lines). 
   The detector noises are listed in Table~\ref{tab:so}. More detailed instrument parameters is given in Appendix Table 3. }
    \label{fig:figure7}
\end{figure*}

==> fig8.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Roman_2.png}
    \caption{Required exposure time ratio between an IFS and an iFTS $\rm{T_{IFS}/{T_{iFTS}}}$ to achieve the same $\rm{S/N}$ with the same resolution for a visible bandpass ($675 - 785 nm$, $R=50$) using Roman space telescope. The required exposure time ratio changes as functions of target distance, star-planet separation, host star temperature and the number of exozodis. We use the Roman CBE level dark current in our simulation.   }
    \label{fig:figure8}
\end{figure*}

==> figA1.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{sampling.png}
    \caption{The sampling effect of interferogram. (a) Original spectrum. (b) Original spectrum and its mirror image. (c) Spectrum replications at Nyquist sample rate $\Delta x=\frac{1}{2\nu_{max}}$. (d) Band-limited spectrum centered at $\nu_{c}$ with bandwidth of $B$ and its mirror image. (e) The replications of band-limited spectrum at sample rate $\nu_{s} = \frac{2\nu_{c}-B}{2}$. (f) The replications of band-limited spectrum at sample rate $\frac{2\nu_{c}+B}{3} <\nu_{s} <\frac{2\nu_{c}-B}{2}$. (g) The replications of band-limited spectrum at sample rate $\nu_{s} = \frac{2\nu_{c}+B}{3}$.     }
    \label{fig:figurea1}
\end{figure*}

==> figA6.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/LUVOIRA_3.png}
    \caption{Same with Figure~\ref{fig:figure11} but for LUVOIR A  }
    \label{fig:figurea6}
\end{figure*}

==> table2_2.tex <==
\begin{longrotatetable}
\begin{deluxetable}{lllllllll}
\tablecaption{Simulation Overview}\label{tab:so}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{\colhead{Simulation} &\colhead{Target}& \colhead{ Diameter} & \colhead{$\tau_{\rm{core}}^{1}$}&\colhead{$\tau_{\rm{optical}}^{2}$} &\colhead{$n_{\rm{pix}}$^{3}} & \colhead{Resolution} &\colhead{VIS detector noise^{4}}& \colhead{NIR detector noise^{4}} }
\startdata
\rule{0pt}{30pt} 
1(a). \makecell{General\\+coronagraph} &\makecell{Earth\\Twin} &2-15 m  & $10\%$& \makecell{ $\rm{VIS}:15\%\\ \rm{NIR}:\ 30\%$}  &\makecell{ $\rm{VIS}:6\\ \rm{NIR}:\ 4$}&\makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 70$}& \makecell[l]{$\rm{i_{d}:0.1\sim3.4\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\ $\rm{q_{cic}:0.0013 e^{-}pix^{-1}frame^{-1}}$ } &  \makecell[l]{$\rm{i_{d}:6.84\  e^{-}pix^{-1}hr^{-1}}$\\$\rm{i_{r}: 0.1\sim 1.8  e^{-}pix^{-1}frame^{-1}}\\ (t_{\rm{frm}}=100s)$\\ $\rm{q_{cic}:0}$} \\
\rule{0pt}{30pt}
1(b). \makecell{General\\+starshade} & \makecell{Earth\\Twin} &2-15 m  & $10\%$& \makecell{ $\rm{VIS}:15\%\\ \rm{NIR}:\ 30\%$} &\makecell{ $\rm{VIS}:18\\ \rm{NIR}:\ 12$} &\makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 70$}&\makecell[l]{$\rm{i_{d}:0.1\sim3.4\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\ $\rm{q_{cic}:0.0013 e^{-}pix^{-1}frame^{-1}}$ } &  \makecell[l]{$\rm{i_{d}:6.84\  e^{-}pix^{-1}hr^{-1}}$\\$\rm{i_{r}: 0.1\sim 1.8  e^{-}pix^{-1}frame^{-1}}\\ (t_{\rm{frm}}=100s)$\\ $\rm{q_{cic}:0}$} \\
\rule{0pt}{30pt}
2. \makecell{Roman\\+coronagraph} & \makecell{Jupiter\\Twin} & 2.37 m & $3\%$& $\rm{VIS}:38\%$ &\makecell{ $\rm{VIS}:6\\ \rm{NIR}:\ 4$}&$\rm{VIS}:140$ & \makecell[l]{$\rm{i_{d}:0.77/1.04/3.37\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\$\rm{q_{cic}:0.01 e^{-}pix^{-1}frame^{-1}}$}&  \makecell[l]{—— } \\
\rule{0pt}{30pt}
3(a). \makecell{HabEx\\ + starshade \\+ current detector \\noise } &\makecell{Earth\\Twin} & 4 m &$69\%$& \makecell{ $\rm{VIS}:30\%\\ \rm{NIR}:\ 35\%$} &\makecell{ $\rm{VIS}:18\\ \rm{NIR}:\ 12$} &\makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 40$}& \makecell[l]{$\rm{i_{d}:0.77\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\$\rm{q_{cic}: 0.01 \ e^{-}pix^{-1}frame^{-1}}$ }   &  \makecell[l]{$\rm{i_{d}:6.84\  e^{-}pix^{-1}hr^{-1}}$\\$\rm{i_{r}:5.9\ e^{-}pix^{-1}frame^{-1}}\\(t_{\rm{frm}}=1000s)$\\ $\rm{q_{cic}:0}$ } \\
\rule{0pt}{30pt}
3(b). \makecell{HabEx\\ + starshade \\+ current detector \\noise } &\makecell{Earth\\Twin} & 4 m &$69\%$& \makecell{ $\rm{VIS}:30\%\\ \rm{NIR}:\ 35\%$} &\makecell{ $\rm{VIS}:18\\ \rm{NIR}:\ 12$} & \makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 40$}&\makecell[l]{$\rm{i_{d}:0.1\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\$\rm{q_{cic}:  0.0013\ e^{-}pix^{-1}frame^{-1}}$ }   &  \makecell[l]{$\rm{i_{d}:5.4\  e^{-}pix^{-1}hr^{-1}}$\\   $\rm{i_{r}: 0.1\ e^{-}pix^{-1}frame^{-1}}\\(t_{\rm{frm}}=100s)$ \\ $\rm{q_{cic}:0}$ } \\
\rule{0pt}{30pt}
\enddata
\tablenotetext{1}{$\tau_{core}$ is the core throughput of coronagraph or starshade, not including optical throughput due to other optical opponents and detector quantum efficiency. }
\tablenotetext{2}{$\tau_{\rm{optical}}$ is the throughput of optical component of the system.}
\tablenotetext{3}{$n_{\rm{pix}}$ is the number pf pixels contributing to one spectral element in IFS simulation.}
\tablenotetext{4}{$i_{d}$: dark current count rate, $i_{c}$: readout noise count rate, $q_{cic}$: clock induced charge, $\rm{t_{frm}}$: integration time per frame.}
\end{deluxetable}
\end{longrotatetable}

\section{Spectrograph Simulator}
\subsection{iFTS numerical simulator}\label{sec:methord}

\input{FTSsimu}

This section describes the iFTS simulation module employed to simulate the spectral observation of an iFTS, with the aim of performing a detailed analysis of the error budget of an iFTS. Figure~\ref{fig:FTSsimu} illustrates an example simulation of an $\rm{O_{2}}$ line in the optical bandpass from 600 nm to 800 nm, obtained from an Earth twin situated 10 pc away. The presented simulations only involve the simplest cases of a purely planet spectrum as an example, and the complete simulation framework with astrophysical backgrounds will be explained in section~\ref{sec:CMW}. 


Figure~\ref{fig:FTSsimu} (a)-(c) present the input spectrum $S_{in}(\nu)$, exposure time $T(\delta)$ at every scanning step $\delta$ and the instrument line spread function (ILS), respectively. The input spectrum is presented as a function of wavenumber $\nu$ in units of $nm^{-1}$ for comparison with the output spectra obtained from the Fourier transform. We assign constant exposure times at every step with a boxcar apodization function. Our FTS simulation is capable of implementing various apodization functions, such as triangle or Hamming functions, which exhibit slightly different ILS (see Appendix X). The ILS of the boxcar function is a \textit{sinc} function shown in panel (c). The effective width of the \textit{sinc} function is determined by the maximum OPD $L$. We choose the maximum scanning position $L$ based on the wavenumber in the middle of the bandpass $\nu_{\rm{mid}}$ and desired resolution $R$. 
\begin{equation}
    \rm{\Delta \nu_{ILS} = \frac{1.206}{2L}} = \frac{\nu_{mid}}{R}
\end{equation}

Figure~\ref{fig:FTSsimu} (d)-(f) display the signal, noise and signal-to-noise ratios of simulated interferogram. The iFTS simulator splits the input spectrum into two beams and computes the interfered intensity at two cameras by scanning a range of optical path differences between them. We also add detector noise and photon noise at every step. The intensity at the two outputs are 
 
\begin{equation}
    I_{+}(\delta)=T(\delta)\sum{\frac{S_{in}(\nu)}{2}(1+\cos{2\pi \nu \delta)}}\Delta \nu +I_{\rm{FTS}}T(\delta)
\end{equation}    

\begin{equation}
    I_{-}(\delta)=T(\delta)\sum{\frac{S_{in}(\nu)}{2}(1-\cos{2\pi \nu \delta)}}\Delta \nu +I_{\rm{FTS}}T(\delta)
\end{equation}
We obtained the interferogram from the difference between $I_{1}$ and $I_{2}$. The interferogram is double-sided and symmetry along the zero optical path difference.

\begin{equation}
   I_{\Delta}(\delta) =I_{+}(\delta)-I_{-}(\delta) = T(\delta)\sum{S_{in}(\nu)\cos{2\pi \nu \delta}}\Delta \nu 
\end{equation}
Panel (d) shows that the sum of simulated intensities at the two outputs is equal to the sum of all photons entering the spectrograph, plus noise from the detectors.
\begin{equation}
    I_{\sum}(\delta)=I_{+}(\delta)+I_{-}(\delta) = T(\delta)\sum{S_{in}(\nu)\Delta \nu + I_{\rm{FTS}}T(\delta)
\end{equation}

In panel (e), we can see that the sum of $I_{1}$ and $I_{2}$ has the same noise as the difference between the two outputs, that is the square root of the total counts:
\begin{equation}\label{eq:sigmaFTS}
    \sigma_{ I_{\Delta}(\delta)}=\sigma_{I_{\sum}(\delta)} = \sqrt{T(\delta)\sum{S_{in}(\nu)\Delta \nu + I_{\rm{FTS}}T(\delta)}}
\end{equation}

The first term inside the square root of  Eq.~\ref{eq:sigmaFTS} is the photon noise, and the second term is the detector noise. 

Figure~\ref{fig:FTSsimu} (g)-(i) display the output spectra from the FTS simulator. We perform the Fourier transform to the simulated interferogram $ I_{\Delta}(\delta)$ and take the real part as the output spectra. The Fast Fourier Transform (FFT) of a real-valued signal, like the two-sided interferogram, is conjugate symmetric. So we obtain symmetric spectra in the positive and negative wavenumbers. The amplitude of the output spectra are half of the input spectra times ILS width and the total exposure time $T_{\rm{tot}}$. So the spectral noise is
\begin{equation}
\begin{split}
    S_{o,\rm{FTS}}(\nu) & = \sum I_{\Delta}(\delta) cos(-2\pi \nu \delta)\Delta \delta \\
        & = \frac{S_{in}(\nu) \Delta \nu_{\rm{ILS}} T_{\rm{tot}}}{2}
\end{split}
\end{equation}

Figure~\ref{fig:FTSsimu} (j)-(k) show the noise of our output spectra, which is white noise independent of the wavenumbers. The variance of the spectral noise is half of the total variance of the interferogram, as we discarded the imaginary part of the FFT output.
\begin{equation}
   \sigma[S_{o,\rm{FTS}}] = \sqrt{\frac{T_{\rm{tot}}\sum{S_{in}(\nu)\Delta \nu +  I_{\rm{FTS}}}T_{\rm{tot}}}{2}}
\end{equation}

Panels (m) - (o) present the signal-to-noise ratio of our output spectra. It can be described by 
\begin{equation}
    \rm{SNR_{FTS}}= \frac{S_{in}(\nu) \Delta \nu_{\rm{ILS}} T_{\rm{tot}}}{\sqrt{2[T_{\rm{tot}}\sum{S_{in}(\nu)\Delta \nu +  I_{\rm{FTS}}}T_{\rm{tot}}]}}
\end{equation}

We present the detailed derivation of FTS SNR in the appendix\textcolor{red}{What happened to this?}~\ref{sec:dde}. \cite{Treffers1977} derived the SNR for one-port FTS scale with $\sqrt{\frac{T_{tot}}{4}}$. If we time his analytical model with a factor of 2 to account for the difference between one-port and two-port FTS, we will get consistent  SNR calculation for our simulations. However, we simulated signal-to-noise ratios (SNRs) are $\sqrt{2}$ times smaller than the values predicted by analytical models from \cite{bennett1999critical} (Eqn. 26 in his paper) when using the same parameters. \cite{bennett1999critical} states that the statistical noise can be reduced by a factor of $\sqrt{2}$ by scanning one-side interferograms instead of double-sided ones. However, this is not reproduced this in numerical simulations as the spectral noise does not depend on the number of scanning steps. The time at each step is usually much longer than the time per frame because of the need to avoid cosmic ray saturation. Thus, we take multiple frames at each step, and the total number of frames is only determined by the total exposure time and the time per frame. The difference means that an iFTS needs double the exposure time to achieve a given SNR than previously predicted. Furthermore, it is not feasible to improve the SNR in our simulations by combining the spectra in negative and positive wavenumbers because the two spectra are conjugate symmetric and not independent. The exposure time for directly characterizing exoplanet spectra is usually over hundreds or thousands of hours, depending on target properties and the instrument parameters \cite{Robinson2016, Lacy2019}. Thus, the significant discrepancy will influence our main conclusions regarding comparing an iFTS and an IFS for exoplanet spectroscopy.
\subsection{IFS numerical simulator}

Figure~\ref{fig:IFSsimu} presents the IFS simulation results. Panel (a) is the input spectra as the function of wavelength. We clipped the spectra into several spectral elements and the width of each elements depends on the resolution $R$: $\Delta \lambda = \frac{\lambda}{R}$. We then integrate the spectra in each element and add the detector noise. 
\begin{equation}
    S_{\rm{o,IFS}}(\lambda) = S_{in}(\lambda)* \Delta \lambda * T_{tot} 
\end{equation}
The noise is the square root of the photon counts per spectral element
\begin{equation}\label{eq:IFSsigma}
    \sigma[S_{o,\rm{IFS}}] = \sqrt{S_{in}(\lambda)* \Delta \lambda * T_{tot} + I_{\rm{IFS}}T_{\rm{tot}}}
\end{equation}

The first term in Eq.~\ref{eq:IFSsigma} is the photo noise. Compared to an iFTS, an IFS has smaller photon noise as it integrate the photons from every elements whereas an iFTS integrate photons from the entire bandpass. But an IFS may suffer more detector noise with $I_{\rm{IFS}}>I_{\rm{iFTS}}$ Therefore, the SNR for an IFS is 
\begin{equation}
    \rm{SNR}_{\rm{IFS}}=\frac{S_{in}(\lambda) \Delta \lambda  T_{tot} }{\sqrt{S_{in}(\lambda) \Delta \lambda  T_{tot} + I_{\rm{IFS}}T_{\rm{tot}}}}
\end{equation}

To make sure our models produces reasonable outputs, we used our simulator to reproduce the IFS simulations from \cite{Robinson2016} and \cite{Lacy2019} and obtained values for the planet photon flux and noise count rate matching theirs within $5\%$

\input{IFSsimu}

==> table2old.tex <==
\textbf{\begin{deluxetable*}{lllllllll}
\tablecaption{Simulation Overview}\label{tab:so}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{\colhead{Simulation} &\colhead{Target}& \colhead{ Diameter} & \colhead{$\tau_{\rm{core}}^{1}$}&\colhead{$\tau_{\rm{optical}}^{2}$} &\colhead{$n_{\rm{pix}}$^{3}} & \colhead{Resolution} &\colhead{VIS detector noise^{4}}& \colhead{NIR detector noise^{4}} }
\startdata
\rule{0pt}{30pt} 
1(a). \makecell{General\\+coronagraph} &\makecell{Earth\\Twin} &2-15 m  & $10\%$& \makecell{ $\rm{VIS}:15\%\\ \rm{NIR}:\ 30\%$}  &\makecell{ $\rm{VIS}:6\\ \rm{NIR}:\ 4$}&\makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 70$}& \makecell[l]{$\rm{i_{d}:0.1\sim3.4\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\ $\rm{q_{cic}:0.0013 e^{-}pix^{-1}frame^{-1}}$ } &  \makecell[l]{$\rm{i_{d}:6.84\  e^{-}pix^{-1}hr^{-1}}$\\$\rm{i_{r}: 0.1\sim 1.8  e^{-}pix^{-1}frame^{-1}}\\ (t_{\rm{frm}}=100s)$\\ $\rm{q_{cic}:0}$} \\
\rule{0pt}{30pt}
1(b). \makecell{General\\+starshade} & \makecell{Earth\\Twin} &2-15 m  & $10\%$& \makecell{ $\rm{VIS}:15\%\\ \rm{NIR}:\ 30\%$} &\makecell{ $\rm{VIS}:18\\ \rm{NIR}:\ 12$} &\makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 70$}&\makecell[l]{$\rm{i_{d}:0.1\sim3.4\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\ $\rm{q_{cic}:0.0013 e^{-}pix^{-1}frame^{-1}}$ } &  \makecell[l]{$\rm{i_{d}:6.84\  e^{-}pix^{-1}hr^{-1}}$\\$\rm{i_{r}: 0.1\sim 1.8  e^{-}pix^{-1}frame^{-1}}\\ (t_{\rm{frm}}=100s)$\\ $\rm{q_{cic}:0}$} \\
\rule{0pt}{30pt}
2. \makecell{Roman\\+coronagraph} & \makecell{Jupiter\\Twin} & 2.37 m & $3\%$& $\rm{VIS}:38\%$ &\makecell{ $\rm{VIS}:6\\ \rm{NIR}:\ 4$}&$\rm{VIS}:50$ & \makecell[l]{$\rm{i_{d}:0.77/1.04/3.37\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\$\rm{q_{cic}:0.01 e^{-}pix^{-1}frame^{-1}}$}&  \makecell[l]{—— } \\
\rule{0pt}{30pt}
3(a). \makecell{HabEx\\ + starshade \\+ current detector \\noise } &\makecell{Earth\\Twin} & 4 m &$69\%$& \makecell{ $\rm{VIS}:30\%\\ \rm{NIR}:\ 35\%$} &\makecell{ $\rm{VIS}:18\\ \rm{NIR}:\ 12$} &\makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 40$}& \makecell[l]{$\rm{i_{d}:0.77\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\$\rm{q_{cic}: 0.01 \ e^{-}pix^{-1}frame^{-1}}$ }   &  \makecell[l]{$\rm{i_{d}:6.84\  e^{-}pix^{-1}hr^{-1}}$\\$\rm{i_{r}:5.9\ e^{-}pix^{-1}frame^{-1}}\\(t_{\rm{frm}}=1000s)$\\ $\rm{q_{cic}:0}$ } \\
\rule{0pt}{30pt}
3(b). \makecell{HabEx\\ + starshade \\+ current detector \\noise } &\makecell{Earth\\Twin} & 4 m &$69\%$& \makecell{ $\rm{VIS}:30\%\\ \rm{NIR}:\ 35\%$} &\makecell{ $\rm{VIS}:18\\ \rm{NIR}:\ 12$} & \makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 40$}&\makecell[l]{$\rm{i_{d}:0.1\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\$\rm{q_{cic}:  0.0013\ e^{-}pix^{-1}frame^{-1}}$ }   &  \makecell[l]{$\rm{i_{d}:5.4\  e^{-}pix^{-1}hr^{-1}}$\\   $\rm{i_{r}: 0.1\ e^{-}pix^{-1}frame^{-1}}\\(t_{\rm{frm}}=100s)$ \\ $\rm{q_{cic}:0}$ } \\
\rule{0pt}{30pt}
4(a). \makecell{LUVOIR\\ + coronagraph \\+ current detector \\noise }  & \makecell{Earth\\Twin} &15/8 m & $10\%$/$20\%$ & \makecell{ $\rm{VIS}:23.8\%\\ \rm{NIR}:\ 32.5\%$} &\makecell{ $\rm{VIS}:6\\ \rm{NIR}:\ 4$} &\makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 70$}& \makecell[l]{$\rm{i_{d}:0.77\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\$\rm{q_{cic}:0.01\ e^{-}pix^{-1}frame^{-1}}$} &  \makecell[l]{$\rm{i_{d}:6.84\  e^{-}pix^{-1}hr^{-1}}$\\$\rm{i_{r}: 5.9\ e^{-}pix^{-1}frame^{-1}}\\(t_{\rm{frm}}=1000s)$ \\ $\rm{q_{cic}:0}$}  \\
\rule{0pt}{30pt}
4(b). \makecell{LUVOIR\\ + coronagraph \\+ future detector \\noise }  & \makecell{Earth\\Twin} &15/8 m & $10\%$/$20\%$ & \makecell{ $\rm{VIS}:23.8\%\\ \rm{NIR}:\ 32.5\%$} &\makecell{ $\rm{VIS}:6\\ \rm{NIR}:\ 4$} &\makecell{ $\rm{VIS}:140\\ \rm{NIR}:\ 70$}& \makecell[l]{$\rm{i_{d}:0.1\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\$\rm{q_{cic}:0.0013\ e^{-}pix^{-1}frame^{-1}}$} &  \makecell[l]{$\rm{i_{d}:5.4\  e^{-}pix^{-1}hr^{-1}}$\\$\rm{i_{r}: 0.1\ e^{-}pix^{-1}frame^{-1}}\\(t_{\rm{frm}}=100s)$ \\ $\rm{q_{cic}:0}$}  \\
\enddata
\tablenotetext{1}{$\tau_{core}$ is the core throughput of coronagraph or starshade, not including optical throughput due to other optical opponents and detector quantum efficiency. }
\tablenotetext{2}{$\tau_{\rm{optical}}$ is the throughput of optical component of the system.}
\tablenotetext{3}{$n_{\rm{pix}}$ is the number pf pixels contributing to one spectral element in IFS simulation.}
\tablenotetext{4}{$i_{d}$: dark current count rate, $i_{c}$: readout noise count rate, $q_{cic}$: clock induced charge, $\rm{t_{frm}}$: integration time per frame.}
\end{deluxetable*}
}

==> table3.tex <==


\begin{center}
\begin{longtable*}[t]{|l|p{1cm}|c|c|c|}
    \label{table:sim_params}
    \caption{Summary of Instrument Parameters}\\
    \hline
    Parameters & Unit & \multicolumn{1}{c|}{Roman} & \multicolumn{1}{c|}{LUOVIR-A/B} &\multicolumn{1}{c|}{HabEx} \\ \hline
    \endfirsthead
    \hline
    \multicolumn{5}{|c|}{Continued from previous page} \\\hline
    Parameters & Unit & \multicolumn{1}{c|}{Roman} & \multicolumn{1}{c|}{LUOVIR-A/B} &\multicolumn{1}{c|}{HabEX} \\ \hline
    \endhead
    \hline 
    \multicolumn{5}{|c|}{\textit{Continued on next page}} \\\hline
    \endfoot
    \hline
    \endlastfoot
    Telescope Diameter $D$   &  m & \multicolumn{1}{c|}{2.36} & \multicolumn{1}{c|}{15/8}  &\multicolumn{1}{c|}{4} \\\hline
    Collecting Area $A$ &  $\rm{m^{2}}$ & 3.684 &  155/43.8 & 12.6   \\\hline
    VIS Total Bandpass &  $\mu m$ & \multicolumn{1}{c|}{0.575-0.825} &\multicolumn{1}{c|}{0.515-1.03} &\multicolumn{1}{c|}{0.45-0.975}\\\hline
    NIR Total Bandpass &  $\mu m$ & \multicolumn{1}{c|}{—} &\multicolumn{1}{c|}{1.0-2.0} &\multicolumn{1}{c|}{0.975-1.8}\\\hline
    VIS Resolution $R$ & — & \multicolumn{1}{c|}{50}&\multicolumn{1}{c|}{140} &\multicolumn{1}{c|}{140} \\\hline
    NIR Resolution $R$ & — & \multicolumn{1}{c|}{—}&\multicolumn{1}{c|}{70} &\multicolumn{1}{c|}{40} \\\hline
    \multicolumn{5}{|c|}{Coronagraph Architecture}\\\hline
    Raw Contrast $C$ &— &  $2.2\times10^{-9}$ & $1\times10^{-10}$ &$ 1\times10^{-10}$\\\hline
    Coronagraph Throughput $\tau_{c}$ &  $\%$ & 3 &  A:$\le 20$/B:$\le 40$ & $\le 40$   \\\hline
    Optical Throughput $\tau_{optical}$ & \% & 38 & VIS: 23.8 NIR: 32.5 & VIS: 15 NIR: 20\\\hline
    \multicolumn{5}{|c|}{Starshade Architecture}\\\hline
    Raw Contrast  $C$ &— & —   &  —   & $1\times10^{-10}$    \\ \hline
    Starshade Throughput $\tau_{s}$ &  $\%$ & —& — & $\ttilde 69$   \\\hline
    Optical Throughput $\tau_{optical}$ & \% & — & — & VIS: 30 NIR: 35\\\hline
    \multicolumn{5}{|c|}{Detector Parameters}\\\hline
    VIS Dark Current  $D_{e^{-}}$ & \multicolumn{1}{p{1cm}|}{$e^{-}$/pix /hr } &\multicolumn{1}{p{4cm}|}{\begin{itemize}
    \item $\rm{1k\times 1k}$ Roman EMCCD (current best estimate): $0.77$
    \item $\rm{1k\times 1k}$ Roman EMCCD (begin of life requirement): $1.04$
    \item $\rm{1k\times 1k}$ Roman EMCCD (end of life requirement): $3.3$
    \end{itemize}} &  0.1 & $<0.36 $\\ \hline
    \multicolumn{1}{|p{4.3cm}|}{VIS Clock-induced Charge $q_{cic}$}& \multicolumn{1}{p{1cm}|}{$e^{-}$/pix /frame } &\multicolumn{1}{p{4cm}|}{\begin{itemize}
    \item $\rm{1k\times 1k}$ Roman EMCCD (begin of life requirement): 0.01
    \item $\rm{1k\times 1k}$ Roman EMCCD (end of life requirement): 0.02
    \end{itemize}}  &$1.3\times10^{-3}$ &$<3\times10^{-3}$\\  \hline
    NIR Dark Current $D_{e^{-}}$ & \multicolumn{1}{p{1cm}|}{$e^{-}$/pix /hr } &\multicolumn{1}{p{3.9cm}|}{HxRG: $6.84$} &   LMAPD: $5.4$  & LMAPD: $5.4$ \\\hline
    NIR Read Noise $R_{e^{-}}$ & \multicolumn{1}{p{1cm}|}{$e^{-}$/pix /frame }&\multicolumn{1}{p{4cm}|} {HxRG: $5.9$} &   LMAPD: $0.1$  & LMAPD: $0.1$ \\\hline
    Integration Time/Frame & s& 100 & 100/1000 & 100/1000\\\hline
    \multicolumn{5}{|c|}{IFS Parameters}\\\hline
    \multicolumn{1}{|p{4cm}|}{Nyquist wavelength} & nm & 575  & VIS:515/NIR:1000 &VIS:450/NIR:975 \\\hline
    \multicolumn{1}{|p{4cm}|}{Pixel Number/Spectral Element $n_{pix}$} & pix &VIS:6 & VIS:6 NIR:4 &  \makecell[l]{coronagraph VIS:6 NIR:4\\starsahde VIS:18 NIR:12}\\\hline
    \multicolumn{1}{|p{4.7cm}|}{Width of Photometric Aperture X (multiple of $\frac{\lambda}{D}$ )} &  — &1 &1 &1 \\\hline
\end{longtable*}
\end{center}



==> table_2n.tex <==
\begin{deluxetable*}{lccccccc}

\tablecaption{Summary of Instrument Parameters\label{tab:rvs}
}
\tablehead{\colhead{Parameter} & \colhead{Fig.6$\&$7} & \colhead{Fig.8}& \colhead{Fig.9}& \colhead{Fig.10}& \colhead{Fig.11}& \colhead{Fig.12}& \colhead{Fig.13} }
\startdata
 Diameter & \multicolumn{7}{|c}{6 m} \\\hline
 Contrast &  \multicolumn{7}{|c}{$10^{-10}$} \\\hline
 Resolution &  \multicolumn{7}{|c}{VIS: 140; NIR: 70} \\\hline
 Nyquist wavelength & \multicolumn{7}{|c}{VIS: 540 nm; NIR: 1000nm} \\\hline
 Quantum Efficiency $\tau_{\text{QE}}$ &  \multicolumn{7}{|c}{VIS: $80\%(\lambda<700 nm) $ nm; NIR: $80\%$} \\\hline
 Optical throughput $\tau_{\text{optical}}$ & \multicolumn{7}{|c}{VIS: $24\%$; NIR: $32\%$} \\\hline
 Coronagraph throughput $\tau_{\text{core}}$ & $10\%$& $10\%$ & $10\%\sim40\%$& $10\%$&$10\%-40\%$ &$10\%$ &$10\%$ & \\\hline
 IFS $n_{\text{pix}}$ & &  & & & & & & \\\hline
 VIS detector noise &$\rm{i_{d}:0.1\sim3.4\  e^{-}pix^{-1}hr^{-1}}$\\$i_{r}:0$\\ $\rm{q_{cic}:0.01 e^{-}pix^{-1}frame^{-1}}\\(t_{\rm{frm}}=100s)$  &  & & & & & & \\\hline
 NIR detector noise & &  & & & & & & \\\hline
\enddata
\end{deluxetable*}


